Extending a User Interface Prototyping Tool with Automatic MISRA C Code Generation

We are concerned with systems, particularly safety-critical systems, that involve interaction between users and devices, such as the user interface of medical devices. We therefore developed a MISRA C code generator for formal models expressed in the PVSio-web prototyping toolkit. PVSio-web allows developers to rapidly generate realistic interactive prototypes for verifying usability and safety requirements in human-machine interfaces. The visual appearance of the prototypes is based on a picture of a physical device, and the behaviour of the prototype is defined by an executable formal model. Our approach transforms the PVSio-web prototyping tool into a model-based engineering toolkit that, starting from a formally verified user interface design model, will produce MISRA C code that can be compiled and linked into a final product. An initial validation of our tool is presented for the data entry system of an actual medical device.

==> eptcsdata.tex <==
\providecommand{\firstpage}{53}
\providecommand{\publicationstatus}{C. Dubois, P. Masci, D. M\'ery (Eds.): F-IDE 2016\\
EPTCS 240, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.240.4}{10.4204/EPTCS.240.4}}
\pdfoutput=1

